Risk Bounds for Unsupervised Cross-Domain Mapping with IPMs

The recent empirical success of unsupervised cross-domain mapping algorithms, between two domains that share common characteristics, is not well-supported by theoretical justifications. This lacuna is especially troubling, given the clear ambiguity in such mappings. We work with adversarial training methods based on IPMs and derive a novel risk bound, which upper bounds the risk between the learned mapping $h$ and the target mapping $y$, by a sum of three terms: (i) the risk between $h$ and the most distant alternative mapping that was learned by the same cross-domain mapping algorithm, (ii) the minimal discrepancy between the target domain and the domain obtained by applying a hypothesis $h^*$ on the samples of the source domain, where $h^*$ is a hypothesis selectable by the same algorithm. The bound is directly related to Occam's razor and encourages the selection of the minimal architecture that supports a small mapping discrepancy and (iii) an approximation error term that decreases as the complexity of the class of discriminators increases and is empirically shown to be small. The bound leads to multiple algorithmic consequences, including a method for hyperparameters selection and for early stopping in cross-domain mapping GANs. We also demonstrate a novel capability for unsupervised learning of estimating confidence in the mapping of every specific sample.

==> old versions/Experiments.tex <==
\section{Experiments}
\label{sec:experiments}
{\color{red} The experiments presented below are a subset of the experiments presented in ~\citep{galanti2018the,benaim2017maximally}.} 

The first group of experiments is intended to test the validity of the two predictions made {\color{red}in Sec.~\ref{sec:conseq}}. {\sout{in order to give further support to the simplicity hypothesis.}} The next group of experiments are dedicated to  Algs.~\ref{algo:when},~\ref{algo:rtrvl} and~\ref{algo:where}. Finally, we evaluate the success of Alg.~\ref{algo:duallayers} in comparison to the DiscoGAN method of~\cite{pmlr-v70-kim17a}. {\color{red}Additional experiments validating Alg.~\ref{algo:when2} from Appendix~\ref{sec:dualProofExt} are presented in the appendix itself.}

Note that while we develop the theoretical results in the context of \sout{IPMs and WGAN} {\color{red} WGANs and IPMs}, the methods developed are widely applicable. In order to demonstrate this, we run our experiments using a wide variety of GAN variants, including CycleGAN\mbox{~\citep{CycleGAN2017}}, DiscoGAN~\citep{pmlr-v70-kim17a}, DistanceGAN~\citep{distgan}, and UNIT~\citep{liu2017unsupervised}, as well as using WGAN itself. The choice of relying on WGAN in the analysis was made, since it is highly accepted as an effective GAN method and since it is amenable to analysis.


\subsection{Experiments for the Predictions}



% We chose to experiment with the DiscoGAN architecture since it focuses on semantic tasks that contain a lesser component of texture or style transfer. The CycleGAN architecture of~\cite{CycleGAN2017} inherits much from the style transfer architecture of Pix2Pix~\cite{pix2pix}, and the discrepancy term is based on a patch-based analysis, which introduces local constraints that could mask the added freedom introduced by adding layers. In addition, the U-net architecture of ~\cite{unet} used by~\cite{pix2pix} deviates from the connectivity pattern of our model. 

% Experiments in this architecture and with the architecture of DualGAN~\citep{dualgan}, which focuses on tasks similar to CycleGAN, and shares many of the architectural choices,  including U-nets and the use of patches, are left for future work.

\begin{figure}[t]
    \centering
    \begin{minipage}{.5\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figures_celebA_blond/gan_onlyA_to_AB.pdf}
    \end{minipage}%
    \begin{minipage}{0.5\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figures_celebA_blond/gan_onlyB_to_BA.pdf}
    \end{minipage}
    \caption{\label{fig:celebA_blond} {\color{red} Results for the celebA dataset for converting blond to black hair and vice versa, when the mapping is obtained by the GAN loss without additional losses.}}
\end{figure}

\begin{figure}[t]
  \centering
 \includegraphics[width=0.6\linewidth,clip]{figures_2to6/DISCOmale2female.pdf}
  \caption{\label{fig:sw004} {\color{red} Results for CelebA Male to Female transfer for DiscoGAN with varying number of layers of the generator. The best results are obtained for $6$ or $8$ layers. For more than $6$ layers, the alignment is lost.} }
\end{figure}

Prediction 1 states that since the unsupervised mapping methods are aimed at learning minimal complexity low discrepancy functions, GANs are sufficient. In this paper, we mainly focus on a complexity measure that is the minimal number of layers of a neural network that are required in order to compute $h$, where each hidden layer is of size $\in [r_1,r_2]$. In the literature~\citep{CycleGAN2017,pmlr-v70-kim17a}, learning a mapping $h:\mathcal{X}_A\rightarrow \mathcal{X}_B$, based only on the GAN constraint on $B$ {\color{red} (e.g., minimize $\W(h \circ D_A,D_B)$)}, is presented as a failing baseline. In~\citep{dualgan}, among many non-semantic mappings obtained by the GAN baseline, one can find images of GANs that are successful. However, this goes unnoticed.

In order to validate the prediction that a purely GAN based solution is viable, we conducted a series of experiments using the DiscoGAN architecture and GAN loss in the target distribution only. We consider image domains $A$ and $B$, where $\mathcal{X}_A = \mathcal{X}_B = \mathbb{R}^{3\times 64\times 64}$.  

In DiscoGAN, the generator is built of: (i) an encoder consisting of convolutional layers with $4\times 4$ filters, followed by Leaky ReLU activation units and (ii) a decoder consisting of deconvolutional layers with $4\times 4$ filters, followed by a ReLU activation units. Sigmoid is used for the output layer. Between four to five convolutional/deconvolutional layers are used, depending on the domains used in $A$ and $B$ (we match the published code architecture per dataset). The discriminator is similar to the encoder, but has an additional convolutional layer as the first layer and a sigmoid output unit. 

The first set of experiments considers the CelebA face dataset. \sout{Transformations are learned between the subset of images labeled as male and those labeled as female, as well as from blond and black hair.} {\color{red} The results for hair color conversions are shown in} \sout{Fig.~\ref{fig:celebA_gender} and} {\color{red} Fig.~\ref{fig:celebA_blond}} \sout{(resp.)}. It is evident that the output image is closely related to the input images, despite the fact that cycle loss terms were not used.

\sout{In the case of mapping handbags to shoes, as seen in Fig.~\ref{fig:handbagtoshoe}, the GAN does not provide a meaningful solution. However, in the case of edges to shoes and vice versa (Fig.~\ref{fig:edges2shoes}), the GAN solution is successful.}


%\subsubsection{Empirical Validation of Prediction 2}

In Prediction 2, we predict that the selection of the right number of layers is crucial in unsupervised learning. Using fewer layers than needed, will not support the modeling of the target distribution. By contrast, adding superfluous layers would mean that more and more alternative mappings obscure the target transformation. 

In~\citep{pmlr-v70-kim17a}, 8 or 10 layers are employed  (counting both convolution and deconvolution), depending on the experiment. In our experiment, we vary the number of layers and inspect the influence on the results. \sout{The experiment  are also repeated for the Wasserstein GAN loss (using the same architecture, except, for the generator, the last sigmoid layer is removed). }

{\color{red} To see the influence of the number of layers of the generator on the results, we employed the DiscoGAN~\citep{pmlr-v70-kim17a} public implementation and added or removed layers from the generator.}
{\color{red}The experiment was} done on the CelebA dataset for male to female conversion where 8 layers are employed in the experiments of~\citep{pmlr-v70-kim17a}. \sout{Using the public implementation and adding and removing layers. We obtain the results in Figs.~\ref{fig:sw001}--~\ref{fig:sw006} for WGAN and Figs.~\ref{fig:a001}--~\ref{fig:a004} for DiscoGAN.} {\color{red} The results are illustrated in Fig.~\ref{fig:sw004}.} Note that since the encoder and the decoder parts of the learned network are symmetrical, the number of layers is always even. As can be seen, changing the number of layers has a dramatic effect on the results. \sout{For the WGAN case, The best overall results are obtained at 8 layers. Using fewer layers, WGAN often fails to produce images of the desired class. Adding layers, the semantic alignment is lost, as expected.} \sout{For the DiscoGAN case,} The best results are obtained at 6 or 8 layers with 6 having the best alignment and 8 having better discrepancy. The results degrade quickly, as one deviates from the optimal value. Using fewer layers, the GAN fails to produce images of the desired class. Adding layers, the semantic alignment is lost, just as expected.

% {\color{red}To provide a numerical analysis, we employ the VGG descriptor~\citep{Parkhi15} to obtain a measure of both separation accuracy and discrepancy as the number of layers vary. We  check if the identity is preserved post mapping by comparing the VGG face descriptors. One can assume that two matching images will have many similar features and so the VGG representation will be similar. The cosine similarities are used, as is commonly done. As we can see, in the DiscoGAN experiments, the optimal values of the three measurements are obtained for 6 and 8 layers.}

\sout{Additional experiment was conducted in order to verify that these conclusions extend to the CycleGAN architecture of\mbox{~\cite{CycleGAN2017}}. The results are shown in Fig.\mbox{~\ref{fig:aer001}}. As can be seen, running  an experiment on the Aerial images to Maps dataset, we found that 8 layers produce an aligned solution. Using 10 layers produces unaligned map images with low discrepancy. For fewer than 8 layer, the discrepancy is high and the images are not very detailed.} 
% For the Segmentations to Images dataset, we found that 6 layers produce an aligned solution. By increasing the number of layers, we obtain mappings that are less aligned and by decreasing the number of layers we obtain less realistic outputs.

% In the WGAN experiment, we employ the architecture of~\citep{pmlr-v70-kim17a} and vary the number of layers and inspect the influence on the results. For the generator, the architecture is identical while for WGAN's critic, the last sigmoid layer is removed. 
% These experiments were done on the CelebA dataset, obtaining the results in Fig.~\ref{fig:sw001}--~\ref{fig:sw006}. 

% Note that since the encoder and the decoder parts of the learned network are symmetrical, the number of layers is always even. As can be seen, changing the number of layers has a dramatic effect on the results. The best overall results are obtained at 6 layers. Using fewer layers, WGAN often fails to produce images of the desired class. Adding layers, the semantic alignment is lost, as expected.


\sout{Note that\mbox{~\cite{pmlr-v70-kim17a}} have preferred low discrepancy over alignment in their choice. In other words, the selected architecture of size $k=8$ presents acceptable images at the price of lower alignment compared to an architecture of size $k-2$. This is probably a result of ambiguity that is already present at the size $k$ architecture. On the other hand, the smaller architecture of size $k-2$ does not produce images of extremely low discrepancy, and there is no architecture that benefits both, an extremely low discrepancy and high alignment.  This is observed, for example in Fig.~\ref{fig:a001}, where females are translated to males. For 4 layers the discrepancy is too low and the mapping fails to produce images of males. For 6 layers, the discrepancy is relatively low and the alignment is at its highest. For 8 layers, the discrepancy is at its lowest value. Nevertheless, the alignment is worse.}

% While our discrete notion of complexity seems to be highly related to the quality of the results, the norm of the weights do not seem to point to a clear architecture, as shown in Tab.~\ref{tab:a001}(a). Since the table compares the norms of architectures of different sizes, we also approximated the functions using networks of a fixed depth $k=18$ and then measured the norm. These results are presented in Tab.~\ref{tab:a001}(b). In both cases, the optimal depth, which is 6 or 8, does not appear to have a be an optimum in any of the measurements. 

% Prediction 3 states that there are only a handful of DPMs,  except for the identity function. In order to verify it, we trained a DiscoGAN from a distribution $A$ to itself with an added loss of the form $-\sum_{x\in A}|x-h(x)|$. In our experiment, testing network complexities from 2 to 12, we could not find a DPM, see Fig.~\ref{fig:c001} and Tab.~\ref{tab:c001}. For lower complexities, the identity was learned despite the added loss. For higher complexities, the network learned the identity while changing the background color. For even higher complexities, other mapping emerged. However, these mappings did not satisfy the circularity constraint, and are unlikely to be DPMs.
% SAY SOMETHING ABOUT CHANGING BACKGROUND COLOR OF IDENTITYE -> Style Transfer -> More complicated geometric transformation. 




\subsection{Results for Algs.~\ref{algo:when} and~\ref{algo:rtrvl}}


\begin{figure*}[t]
\centering
\hspace{-0.6cm}
  \begin{tabular}{c@{~}c@{~}c}
  \centering{\begin{turn}{90}\;\;\;\;~~~Shoes2Edges\end{turn}}&\includegraphics[width=0.4\linewidth, clip]{figures_per_epoch/shoes_disco_per_epoch.pdf}&%\hspace{-0.4cm} 
\includegraphics[width=0.4\linewidth, clip]{figures_per_epoch/shoes_dist_per_epoch.pdf}\\
& (Alg~\ref{algo:when}, discoGAN)  & (Alg~\ref{algo:when}, distanceGAN) \\
\end{tabular}
\caption{{\color{red}Results of Alg.~\ref{algo:when} for mapping Shoes to Edges. Ground truth errors are in red and bound in black. x-axis is the iteration. y-axis is expected risk. It takes a few epochs for $h_1$ to have a small enough discrepancy, until which the bound is ineffective.}}
  \label{fig:whenMain}
\end{figure*}

We test the two algorithms on two unsupervised alignment methods: DiscoGAN~\citep{pmlr-v70-kim17a} and % CycleGAN~\cite{CycleGAN2017}, and 
DistanceGAN~\citep{distgan}. In DiscoGAN, we train $h_1$ (and $h_2$), using two GANs and two circularity constraints; in DistanceGAN, {\color{red}to train $h_1$ (and $h_2$),} one GAN and one distance correlation loss are used. The published hyperparameters for each dataset are used, except \sout{when applying our model selection method, where we vary the number of layers and} when using Hyperband, where we \sout{also} vary the {\color{red}number of layers, the} learning rate and the batch size. 

Five datasets were used in the experiments: (i) aerial photographs to maps, trained on data scraped from Google Maps~\citep{pix2pix}, (ii) the mapping between photographs from the cityscapes dataset and their per-pixel semantic labels~\citep{Cordts2016Cityscapes}, (iii) architectural photographs to their labels from the CMP Facades dataset~\citep{facades},  (iv) handbag images~\citep{handbag} to their binary edge images, as obtained from the HED edge detector~\citep{hed}, and (v) a similar dataset for the shoe images from~\citep{shoes}.

Throughout the experiments, fixed values are used as the low-discrepancy threshold ($\epsilon_0=0.2$). The tradeoff parameter between the dissimilarity term and the fitting term during the training of $h_2$ is set, per dataset, to be the maximal value, such that the fitting of $h_2$ provides a solution that has a discrepancy lower than the threshold. This is done once, for the default parameters of $h_1$, as given in the original DiscoGAN and DistanceGAN~\citep{pmlr-v70-kim17a,distgan}.

The results of all experiments are summarized in Tab.~\ref{tab:mainresults}, which presents the correlation and p-value between the ground truth error, as a function of the independent variable, and the bound. The independent variable is either the training epoch or the sample, depending on the algorithm tested. For example, in Alg.~\ref{algo:when} we wish to decide on the best epoch, the independent variable is the training epoch. A high correlation (low p-value) between the bound and the ground truth error, both as a function of the number of layers, indicates the validity of the bound and the utility of the algorithm. Similar correlations are shown with the GAN losses and the reconstruction losses (DiscoGAN) or the distance correlation loss (DistanceGAN), in order to demonstrate that these are much less correlated with the ground truth error. In Fig.~\ref{fig:whenMain}, we omit the other scores in order to reduce clutter.

\begin{table*}[t]
\centering
\begin{small}
\caption{Pearson correlations and the corresponding p-values (in parentheses) of the ground truth error with: (i) the bound, (ii) the GAN losses, and (iii) the circularity losses or (iv) the distance correlation loss. %Note that the p-value is a function of both the correlation strength and the number of samples, which is larger for Alg.~2. 
$^{*}$The cycle loss $A\rightarrow B\rightarrow A$ is shown for DiscoGAN and the distance correlation loss is shown for DistanceGAN.}
\label{tab:mainresults}
\resizebox{0.99000995\textwidth}{!}{% <------ Don't forget this %
\begin{tabular}{l@{~~}l@{~~}llcccc}
\toprule
Alg. & Method & Dataset & Bound & $GAN_A$ & $GAN_B$ & $Cycle_A/\mathcal{L}_D$$^{*}$ & $Cycle_B$ \\
\midrule

Alg.~\ref{algo:when}  & Disco-    & Shoes2Edges    & {\bf 1.00} (\textless1E-16)          & -0.15 (3E-03)         & -0.28 (1E-08)  & 0.76(\textless1E-16)           & 0.79(\textless1E-16)   \\
                             &  GAN~\cite{pmlr-v70-kim17a}          &&&&&\\ %& Bags2Edges &        {\bf 1.00}	(\textless1E-16)& -0.26 (6E-11) &	-0.57 (\textless1E-16) &	0.85 (\textless1E-16) &	0.84 (\textless1E-16)           \\
                             %&             & Cityscapes        & {\bf 0.94}   (\textless1E-16)        & -0.66 (\textless1E-16)          & -0.69 (\textless1E-16)          & -0.26  (1E-07)        & 0.80 (\textless1E-16)   \\
                             %&             & Facades           & {\bf 0.85}  (\textless1E-16)         & -0.46  (\textless1E-16)        & 0.66 (\textless1E-16)           & 0.92 (\textless1E-16)          & 0.66  (\textless1E-16)         \\
                             %&             & Maps              & {\bf 1.00}     (\textless1E-16)      & -0.81 (\textless1E-16)          & 0.58  (\textless1E-16)         & 0.20   (9E-05)        & -0.14   (5E-03)       \\
                             %& Distance- & Shoes2Edges    &           {\bf 0.98} (\textless1E-16)	& - &	-0.25	(2E-16) & -0.14 (1E-05)	    &       -         \\
                             %&  GAN~\cite{distgan}           & Bags2Edges &            {\bf 0.93} (\textless1E-16) & - &	-0.08 (2E-02) &	0.34	(\textless1E-16)     &        -        \\
                             
                             %&             & Cityscapes        & {\bf 0.59}  (\textless1E-16)         & -          & 0.22   (1E-11)        & -0.41   (\textless1E-16)        &          -      \\
                             %&             & Facades           & {\bf 0.48}    (\textless1E-16)       & -        & 0.03  (5E-01)         & -0.01   (9E-01)       &        -        \\
                             %&             & Maps              & {\bf 1.00}    (\textless1E-16)       & -         & -0.73  (\textless1E-16)         & 0.39   (4E-16)        &      -          \\


\midrule
Alg.~\ref{algo:where} & Disco-    & Shoes2Edges    & {\bf 0.92}  (\textless1E-16)         & -0.12 (5E-01)         & 0.02  (9E-01)         & 0.29  (6E-02)         & 0.15    (4E-01)       \\
                             &       GAN~\cite{pmlr-v70-kim17a}      & Bags2Edges & {\bf 0.96}  (\textless1E-16)           & 0.25  (1E-01)         & 0.08   (6E-01)        & 0.08   (6E-01)        & 0.05  (7E-01)         \\
                             &             & Cityscapes        &        {\bf 0.78} (4E-04) &	0.24 (4E-01)	& -0.16 (6E-01) &	-0.04 (9E-01) &	0.03 (9E-01)    \\
                             &             & Facades           & {\bf 0.80}   (6E-10)        & 0.13   (4E-01)        & 0.16     (3E-01)      & 0.20    (2E-01)       & 0.09     (5E-01)      \\
                             &             & Maps             & {\bf 0.66}    (1E-03)       & 0.08   (7E-01)        & 0.12    (6E-01)       & 0.17   (5E-01)        & -0.25  (3E-01)        \\
                             & Distance- & Shoes2Edges    & {\bf 0.98}    (\textless1E-16)        & -     & -0.05   (7E-01)       & 0.84  (\textless1E-16)         & -               \\
                             &     GAN~\cite{distgan}        & Bags2Edges &  {\bf 0.92}      (\textless1E-16)      & -        & -0.28  (2E-01)        & 0.45    (3E-02)       &         -       \\
                             &             & Cityscapes        &   {\bf 0.51} (4E-04)            &        -        &   0.10 (5E-01)             &        0.28 (2E-2)        &           -     \\
                             &             & Facades           & {\bf 0.72}    (\textless1E-16)        & -      & -0.01    (1E00)      & 0.08  (6E-01)         &   -        \\
                             &             & Maps              &  {\bf 0.94}   (1E-06)        & -    & 0.20    (2E-01)       & 0.30  (6E-02)          &       -  \\
%1    & DiscoGAN & Facades     & %\ref{fig:somefig}(a) & 
%{{\bf \begin{tabular}[c]{@{}l@{}}0.77\\ 2.2E-6\end{tabular}}} & \begin{tabular}[c]{@{}l@{}}0.27\\ 1.2E-1\end{tabular}          &         &     %      &           \\
\bottomrule
\end{tabular}}
\end{small}
\end{table*}



\paragraph{Stopping Criterion (Alg.~\ref{algo:when})} For testing the stopping criterion suggested in Alg.~\ref{algo:when}, we compared, at each time point, two scores that are averaged over all training samples: $||h_1(x) - h_2(x)||$, which is our bound in Eq.~\ref{eq:boundEps0} (excluding the $+\epsilon_0$ term), and the ground truth error $||h_1(x) - y(x)||$, where $y(x)$ is the ground truth image that matches $x$ in domain $B$. 

\sout{Note that similar to the experiments with ground truth in the literature\mbox{~\citep{pmlr-v70-kim17a,CycleGAN2017,distgan}}, the ground truth error is measured in the label space and not in the image domain. The mapping in the other direction $y$ is not one to one.}

The results are depicted in the main results table (Tab.~\ref{tab:mainresults}) as well as in Fig.~\ref{fig:whenMain} for both DiscoGAN (first column) and DistanceGAN (second column). {\color{red} The results for Shoes to Edges are depicted in Fig.~\ref{fig:whenMain}.} As can be seen, there is an excellent match between the mean ground truth error of the learned mapping $h_1$ and the predicted error. No such level of correlation is present when considering the GAN losses or the reconstruction losses (for DiscoGAN), or the distance correlation loss of DistanceGAN. Specifically, the very low p-values in the first column of Tab.~\ref{tab:mainresults} show that there is a clear correlation between the ground truth error and our bound for all datasets. For the other columns, the values in question are chosen to be the losses used for $h_1$. The lower scores in these columns show that none of these values are as correlated with the ground truth error, and so cannot be used to estimate this error.

In the experiment of Alg.~\ref{algo:when} for DiscoGAN, which has a large number of sample points, the cycle from $B$ to $A$ and back to $B$ is significantly correlated with the ground truth error with very low p-values in four out of five datasets. However, its correlation is significantly lower than that of our bound.

\sout{In Fig.~\ref{fig:when}, the Facades graph shows a different behavior than the other graphs. This is because the Facades dataset is inherently ambiguous and presents multiple possible mappings from $A$ to $B$. Each mapping satisfies the Occam's razor property separately. }

{\color{red} These results also demonstrate the tightness of the bound in Thm.~\ref{thm:corBoundGEN}. As can be seen, the bound is tight (close to the test error) and highly correlated with the test error.}



\paragraph{Selecting Architecture with the Modified Hyperband Algorithm} Our bound is used in Sec.~\ref{sec:hyperband} to create an unsupervised variant of the Hyperband method. In addition to selecting the architecture, this allows for the optimization of multiple hyperparameters at once, while enjoying the efficient search strategy of the Hyperband method~\citep{hyperband}. 

Fig.~\ref{fig:hyperband} demonstrates the applicability of our unsupervised Hyperband-based method for different datasets, employing both DiscoGAN and DistanceGAN. The graphs show the error and the bound obtained for the selected configuration after up to 35 Hyperband iterations. As can be seen, in all cases, the method is able to recover a configuration that is significantly better than what is recovered, when only optimizing for the number of layers. To further demonstrate the generality of our method, we applied it on the UNIT~\citep{liu2017unsupervised} architecture. Specifically, for DiscoGAN and DistanceGAN, we optimize the number of encoder and decoder layers, batch size and learning rate, while for UNIT, we optimize for the number of encoder and decoder layers, number of resnet layers and learning rate. Fig.~\ref{fig:hyperband_unit} and Tab.~\ref{fig:hyperband}(b) show the convergence on the Hyperband method. 

\begin{figure*}[t]
\begin{tabular}{c@{~}c}
\multicolumn{2}{c}{\includegraphics[width=1.0\linewidth, clip]{graphs_hyperband/units_maps.pdf}}\\
~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~(a) & ~~~~(b)\\
\end{tabular}
\caption{{\color{red} Applying unsupervised Hyperband for selecting the best configuration for UNIT for the Maps dataset. The $x$-axis is the iteration count and the $y$-axis is the error/bound value of the selected configuration. (a) blue and orange lines are bound and ground truth error as in Fig.~\ref{fig:hyperband}. (b) Images produced for three different configurations, as indicated on the plot in (a).} }
 \label{fig:hyperband_unit}
\end{figure*}

\begin{figure*}[t]
\centering
  %\begin{tabular}{ccccc}
%\hspace{-0.4cm}\includegraphics[width=0.20\linewidth, clip]{graphs_hyperband/maps_new.png}&
%\includegraphics[width=0.20\linewidth, clip]{graphs_hyperband/cityscapes_new.png}&
%\includegraphics[width=0.20\linewidth, clip]{graphs_hyperband/facades_new.png}&
% \includegraphics[width=0.20\linewidth, clip]{graphs_hyperband/shoes_new.png}&
%  \includegraphics[width=0.20\linewidth, clip]{graphs_hyperband/handbags_new.png}\\
%\hspace{-0.4cm}\includegraphics[width=0.20\linewidth, clip]{graphs_hyperband/distance_maps_new.png}&
%\includegraphics[width=0.20\linewidth, clip]{graphs_hyperband/distance_cityscapes_new.png}&
% TODO!!!
%\includegraphics[width=0.20\linewidth, clip]{graphs_hyperband/distance_cityscapes_new.png}&
% \includegraphics[width=0.20\linewidth, clip]{graphs_hyperband/distance_shoes_new.png}&
 % \includegraphics[width=0.20\linewidth, clip]{graphs_hyperband/distance_handbags_new.png}\\
 
 %(Maps) & (Cityscapes) & (Facades) & (Shoes2Edges) & (Handbags2Edges)\\
%\end{tabular}
\vspace{-2cm}
\begin{minipage}{0.656772\textwidth}
\centering
\begin{tabular}{c@{~}c@{~}c}
\centering{\begin{small}\begin{turn}{90}\;\;\;\;\;\; \hspace{3mm} Maps\end{turn}\end{small}}&
\includegraphics[width=0.482\linewidth, clip]{graphs_hyperband/maps_new.png}\vspace{-2mm}&
\includegraphics[width=0.482\linewidth, clip]{graphs_hyperband/distance_maps_new.png}\vspace{-2mm}\\
\centering{\begin{small}\begin{turn}{90}\;\;\;\;\;\; \hspace{1mm}Cityscapes\end{turn}\end{small}}&
\includegraphics[width=0.482\linewidth, clip]{graphs_hyperband/cityscapes_new.png}\vspace{-2mm}&
\includegraphics[width=0.482\linewidth, clip]{graphs_hyperband/distance_cityscapes_new.png}\vspace{-2mm}\\

\centering{\begin{small}\begin{turn}{90}\;\;\;\;\;\; \hspace{3mm}Facades\end{turn}\end{small}}&
\includegraphics[width=0.482\linewidth, clip]{graphs_hyperband/facades_new.png}\vspace{-2mm}&
\includegraphics[width=0.482\linewidth, clip]{graphs_hyperband/distance_facades_new.png}\vspace{-2mm}\\
\centering{\begin{small}\begin{turn}{90}\;\;\;\;\;\; \hspace{-3mm} Bags2Edges\end{turn}\end{small}}&
\includegraphics[width=0.482\linewidth, clip]{graphs_hyperband/handbags_new.png}\vspace{-2mm}&
\includegraphics[width=0.482\linewidth, clip]{graphs_hyperband/distance_handbags_new.png}\vspace{-2mm}\\

\centering{\begin{small}\begin{turn}{90}\;\;\;\;\;\; Shoes2Edges\end{turn}\end{small}}&
\includegraphics[width=0.482\linewidth, clip]{graphs_hyperband/shoes_new.png}\vspace{-2mm}&
\includegraphics[width=0.482\linewidth, clip]{graphs_hyperband/distance_shoes_new.png}\vspace{-2mm}\\
 \multicolumn{3}{c}{(a)}
  \\
\end{tabular}
  \end{minipage}%
\begin{minipage}{.71\textwidth}
\hspace{0.1mm}
\begin{small}
\resizebox{0.48\textwidth}{!}{% <------ Don't forget this %
\begin{tabular}{l@{~~}ccc}
\toprule
Dataset & Number & Batch & Learning \\
 &  Layers & Size & Rate \\
\midrule
\multicolumn{4}{c}{DiscoGAN~\citep{pmlr-v70-kim17a}}\\
            Shoes2Edges       & 3 & 24 & 0.0008 \\
            Bags2Edges        & 2 & 59 &	0.0010 \\
                                  Cityscapes        & 3 & 27 & 0.0009 \\
                                  Facades           & 3 & 20 & 0.0008 \\
                                  Maps              & 3 & 20 & 0.0005 \\
                                  \multicolumn{4}{c}{DistanceGAN~\citep{distgan}} \\
                             Shoes2Edges       & 3 & 15 & 0.0007 \\
                Bags2Edges        & 3 & 33 &	0.0007 \\
                                  Cityscapes        & 4 & 21 & 0.0006 \\
                                  Facades           & 3 & 8  & 0.0006 \\
                                  Maps              & 3 & 20 & 0.0005 \\     
                                  \toprule
Dataset & \#Layers & \#Res & L.Rate \\
% & Layers & Layers & Rate \\
 \midrule
\multicolumn{4}{c}{UNIT~\citep{liu2017unsupervised}} \\
                                  Maps              & 3 & 1 & 0.0003 \\     
\bottomrule
%\hspace{0.1mm}
%& & &\\
\multicolumn{4}{c}{(b)}
\end{tabular}}
%\end{small}
%\end{minipage}%
%\begin{minipage}{0.656772\textwidth}

\centering
\hspace{0.3mm}
\begin{tabular}{l@{~~}l@{~~~}l}
& {\scriptsize default} & {\scriptsize unsupervised}\\
 & {\scriptsize parameters} & {\scriptsize hyperband} \\
~~~$x$ & {\footnotesize $h_1(x)$} & {\footnotesize $h_1(x)$} \\

\includegraphics[width=0.120\linewidth, clip]{images_hyperband_before/2_B.png}&
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_before/2_BA.png}&
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_after/2_BA.png} \\
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_before/3_B.png}&
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_before/3_BA.png}&
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_after/3_BA.png} \\
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_before/5_B.png}&
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_before/5_BA.png}&
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_after/5_BA.png} \\
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_before/13_B.png}&
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_before/13_BA.png}&
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_after/13_BA.png} \\
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_before/16_B.png}&
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_before/16_BA.png}&
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_after/16_BA.png} \\
 \multicolumn{3}{c}{(c)}
  \\
\end{tabular}
\end{small}
  \end{minipage}%
% (b) \\ 
% \resizebox{0.99000995\textwidth}{!}{% <------ Don't forget this %
% \begin{tabular}{l@{~~}|c|ccc|c|ccc}
% \toprule
% Dataset & Method & Number of Layers & Batch Size & Learning Rate & Method & Number of Layers & Batch Size & Learning Rate \\
% \midrule
% Shoes2Edges &  Disco-       & 3 & 24 & 0.0008  & Dist-                           &  3 & 15 & 0.0007 \\
% Bags2Edges  &  GAN~\cite{pmlr-v70-kim17a}    & 2 & 59 &	0.0010 &   GAN~\cite{distgan}             & 3 & 33 &	0.0007 \\
% Cityscapes &        & 3 & 27 & 0.0009 & & 4 & 21 & 0.0006 \\
% Facades    &       & 3 & 20 & 0.0008 & &      &   &           \\
% Maps       &       & 3 & 20 & 0.0005 &  & 3 & 20 & 0.0005 \\   
% \bottomrule
% \end{tabular}} 
\caption{\small {\color{red}Applying unsupervised hyperband for selecting the best configuration. For DiscoGAN and DistanceGAN, we optimize of the number of encoder and decoder layers, batch size and learning rate, while for UNIT, we optmized for the number of encoder and decoder layers, number of resnet layers and learning rate. (a) For each dataset, the first plot is of DiscoGAN and the second is of DistanceGAN. Hyperband optimizes, according to the bound values indicated in blue. The corresponding ground truth errors are shown in orange. Dotted lines represent the best configuration errors, when varying only the number of layers without hyperband (blue for bound and orange for ground truth error). Each graph shows the error of the best configuration selected by hyperband, as a function the number of hyperband iterations. (b) The corresponding hyperparameters of the best configuration as selected by hyperband. (c) Images produced for DiscoGAN's shoes2edges: 1st column is the input, the 2nd is the result of DiscoGAN's default configuration, 3rd is the result of the configuration  selected by our unsupervised Hyperband.} }
  \label{fig:hyperband}
\end{figure*}



\paragraph{Predicting per-Sample loss with Alg.~\ref{algo:where}} Finally, we consider the per sample loss. %Determining the success of the prediction of a computer vision method for a given sample is often crucial, yet challenging even for supervised methods that predict a single value. 
The results are \sout{reported numerically in Tab.~\ref{tab:mainresults} and} plotted in Fig.~\ref{fig:oneSamp2}. {\color{red}Each point in the plot specifies the evaluation of the bound ($y$-axis) vs. the per-sample error ($x$-axis) of the trained generator $h_1$ for a specific point $x$ in domain $A$. The numbered points in the graph correspond to the samples in (b).} As can be seen, there is a high degree of correlation {\color{red}(the coefficient of determination is large, $R^2=0.9145$)} between the measured bound and the ground truth error. Therefore, our method is \sout{able to reliably predict} {\color{red} a reliable predictor of} the per-sample success of a multivariate mapping learned in a fully unsupervised manner. 

\begin{figure*}[t]
  \centering
  \begin{tabular}{c@{~~~~~~~~~~}c}
\includegraphics[width=0.425\linewidth, clip]
{graphs_per_sample/handbags2edges_plot__2_.png}&
\includegraphics[width=0.24\linewidth, clip]{graphs_per_sample/images_edges2handbags_rr.png}\\
(a) & (b) \\
\end{tabular}
\caption{{\color{red} Results of Alg.~\ref{algo:where} on DiscoGAN for Handbags2Edges. (a) The ground truth errors ($x$-axis) vs. the bound per point ($y$-axis) are shown. %\sout{This is the same as Fig.~\ref{fig:alg3_1} top right plot with added information identifying specific points.}
(b) The source ($x$), ground truth ($y(x)$) and mapping ($h_1(x)$) of the marked points.}}
\label{fig:oneSamp2}
\end{figure*}

\sout{This correlation also seems to hold when considering the time axis, i.e., we can combine Alg.~\ref{algo:when}~and Alg.~\ref{algo:where} and select the stopping epoch that is best for a specific sample. The results are shown in Fig.~\ref{fig:alg3_1}.}


\subsection{Results for Alg.~\ref{algo:duallayers}}


\begin{figure}[t]
    \centering
    \begin{minipage}{.5\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figures_dual/DUALmale2femaleS.pdf}
    \end{minipage}%
    \begin{minipage}{0.5\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figures_dual/DUALedges2shoesS.pdf}
    \end{minipage}
    \caption{\label{fig:dual} {\color{red} Results for Alg.~\ref{algo:duallayers} on Male2Female and Edges2Shoes datasets for mapping Male to Female (and for mapping Edges to Shoes, resp.). Shown are a minimal complexity mapping $g$ that has low discrepancy, and various mappings $h$ obtained by the method.}}
\end{figure}
 

The goal of Alg.~\ref{algo:duallayers} is to find a well-aligned solution with higher complexity than the minimal solution and a potentially smaller discrepancy. It has two stages. In the first one, $k_1$, which is the minimal complexity that leads to a low discrepancy, is identified. This follows a set of experiments that are similar to the one that is captured, for example, by Fig.~\ref{pred2}. To demonstrate robustness, we select a single value of $k_1$ across all experiments. Specifically, we use $k_1=6$, which, as discussed above, typically leads to a low (but not very low) discrepancy, while the alignment is still unambiguous.  

Once $g$ is trained, we proceed to the next step of optimizing a second network of complexity $k_2$. Note that while the first function ($g$) uses the complete DiscoGAN architecture, the second network ($h$) only employs a one-directional mapping, since alignment is obtained by $g$.

\sout{Figs.~\ref{fig:dual0}--~\ref{fig:dual5} depict} {\color{red} We conducted the experiments on the CelebA dataset for Male to Female and Edges to Shoes conversions. Fig.~\ref{fig:dual} depicts} the obtained results, for a varying number of layers. First, the result obtained by the DiscoGAN method with $k_1$ is displayed. The results of applying Alg.~\ref{algo:duallayers} are then displayed for a varying $k_2$.

As can be seen, our algorithm leads to more sophisticated mappings. \cite{pmlr-v70-kim17a} have noted that their solutions are, at many times, related to texture or style transfer and, for example, geometric transformations are not well-captured. The new method is able to better capture such complex transformations. Consider the case of mapping Male to Female in Fig.~\ref{fig:dual}, first row. A man with a beard is mapped to a female image. While for $g$ the beard is still somewhat present, it is not so for $h$ with $k_2>k_1$. \sout{On the female to male mappings in Fig.~\ref{fig:dual1}, it is evident in most mappings that $g$ produces a more blurred image, while $h$ is more coherent for $k_2>k_1$. 
Another example is in the blond to black hair mapping in Fig.~\ref{fig:dual1}. In the 5th row, the style transfer nature of $g$ is evident, since it maps a red object behind the head together with the whole blond hair, producing an unrealistic black hair. The $h$ of complexity $k_2=8$ is able to separate that object from the hair, and in $k_2>8$ it produces realistic looking black hair. This kind of transformation requires more than a simple style transfer.} For the Edges to Shoes \sout{and edges to handbags mappings of Fig.~\ref{fig:dual4} and Fig.~\ref{fig:dual5}} {\color{red} mapping of Fig.~\ref{fig:dual}}, while the general structure is clearly present, it is significantly sharpened by mapping $h$ with $k_2>k_1$. 

\sout{For the face datasets, we also employ face descriptors in order to learn whether the mapping is semantic. We can check if the identity is preserved post mapping, by comparing the VGG face descriptors of\mbox{~\cite{Parkhi15}}. One can assume that two matching images that match will have many similar features and so the VGG representation will be similar. The cosine similarities are used, as is commonly done.} 

\sout{In addition, we train a linear classifier in the space of the VGG face descriptors, in order to distinguish between Male/Female, Eyeglasses/No-eyeglasses, and Blond/Black. This allows us to check, beyond discrepancy, that the mapping indeed transforms between the domains. The training samples in domains $A$ and $B$ are used to train this classifier, which is then applied to a set of test images before and after mapping, measuring the accuracy. The higher the accuracy, the better the separation.}

\sout{Tab.~\ref{tab:alg1exp1} presents the results for both the $k_1$ layers network $g$, alternative networks $g$ of higher complexity (shown as baseline only), and the network $h$ trained using Alg.~\ref{algo:duallayers}. 
We expect the alignment of $g$ to be best at complexity $k_1$, and worse due to the loss of discrepancy for alternative network $g$ with complexity $k>k_1$. We expect this loss of alignment to be resolved for networks $h$ trained with Alg.~\ref{algo:duallayers}.}

\sout{In the experiments of black to blond hair and blond to black hair mappings, we note that $h$ with $k_2=8$ has the best descriptor similarity, and very good separation accuracy and discrepancy. Higher values of $k_2$ are best in terms of separation accuracy and discrepancy, but lose somewhat in descriptor similarity. A similar situation occurs for male to female and female to male mappings and in eyeglasses to non-eyeglasses, where $k_2=8$ results in the best similarity score and higher values of $k_2$ result in better separation accuracy and discrepancy. }

\sout{It is interesting to note, that the distance between $g$ and $h$ is also minimal for $k_2=8$. Perhaps, with more effective optimization, higher complexities could also maintain similarity, while delivering lower discrepancies.}



==> old versions/Experiments_clean.tex <==
\section{Experiments}
\label{sec:experiments}
{\color{black} The experiments presented below are a subset of the experiments presented in ~\citep{galanti2018the,benaim2017maximally}.} 

The first group of experiments is intended to test the validity of the two predictions made {\color{black}in Sec.~\ref{sec:conseq}}. The next group of experiments are dedicated to  Algs.~\ref{algo:when},~\ref{algo:rtrvl} and~\ref{algo:where}. Finally, we evaluate the success of Alg.~\ref{algo:duallayers} in comparison to the DiscoGAN method of~\cite{pmlr-v70-kim17a}. {\color{black}Additional experiments validating Alg.~\ref{algo:when2} from Appendix~\ref{sec:dualProofExt} are presented in the appendix itself.}

Note that while we develop the theoretical results in the context of {\color{black} WGANs and IPMs}, the methods developed are widely applicable. In order to demonstrate this, we run our experiments using a wide variety of GAN variants, including CycleGAN\mbox{~\citep{CycleGAN2017}}, DiscoGAN~\citep{pmlr-v70-kim17a}, DistanceGAN~\citep{distgan}, and UNIT~\citep{liu2017unsupervised}, as well as using WGAN itself. The choice of relying on WGAN in the analysis was made, since it is highly accepted as an effective GAN method and since it is amenable to analysis.


\subsection{Experiments for the Predictions}



% We chose to experiment with the DiscoGAN architecture since it focuses on semantic tasks that contain a lesser component of texture or style transfer. The CycleGAN architecture of~\cite{CycleGAN2017} inherits much from the style transfer architecture of Pix2Pix~\cite{pix2pix}, and the discrepancy term is based on a patch-based analysis, which introduces local constraints that could mask the added freedom introduced by adding layers. In addition, the U-net architecture of ~\cite{unet} used by~\cite{pix2pix} deviates from the connectivity pattern of our model. 

% Experiments in this architecture and with the architecture of DualGAN~\citep{dualgan}, which focuses on tasks similar to CycleGAN, and shares many of the architectural choices,  including U-nets and the use of patches, are left for future work.

\begin{figure}[t]
    \centering
    \begin{minipage}{.5\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figures_celebA_blond/gan_onlyA_to_AB.pdf}
    \end{minipage}%
    \begin{minipage}{0.5\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figures_celebA_blond/gan_onlyB_to_BA.pdf}
    \end{minipage}
    \caption{\label{fig:celebA_blond} {\color{black} Results for the celebA dataset for converting blond to black hair and vice versa, when the mapping is obtained by the GAN loss without additional losses.}}
\end{figure}

\begin{figure}[t]
  \centering
 \includegraphics[width=0.6\linewidth,clip]{figures_2to6/DISCOmale2female.pdf}
  \caption{\label{fig:sw004} {\color{black} Results for CelebA Male to Female transfer for DiscoGAN with varying number of layers of the generator. The best results are obtained for $6$ or $8$ layers. For more than $6$ layers, the alignment is lost.} }
\end{figure}

Prediction 1 states that since the unsupervised mapping methods are aimed at learning minimal complexity low discrepancy functions, GANs are sufficient. In this paper, we mainly focus on a complexity measure that is the minimal number of layers of a neural network that are required in order to compute $h$, where each hidden layer is of size $\in [r_1,r_2]$. In the literature~\citep{CycleGAN2017,pmlr-v70-kim17a}, learning a mapping $h:\mathcal{X}_A\rightarrow \mathcal{X}_B$, based only on the GAN constraint on $B$ {\color{black} (e.g., minimize $\W(h \circ D_A,D_B)$)}, is presented as a failing baseline. In~\citep{dualgan}, among many non-semantic mappings obtained by the GAN baseline, one can find images of GANs that are successful. However, this goes unnoticed.

In order to validate the prediction that a purely GAN based solution is viable, we conducted a series of experiments using the DiscoGAN architecture and GAN loss in the target distribution only. We consider image domains $A$ and $B$, where $\mathcal{X}_A = \mathcal{X}_B = \mathbb{R}^{3\times 64\times 64}$.  

In DiscoGAN, the generator is built of: (i) an encoder consisting of convolutional layers with $4\times 4$ filters, followed by Leaky ReLU activation units and (ii) a decoder consisting of deconvolutional layers with $4\times 4$ filters, followed by a ReLU activation units. Sigmoid is used for the output layer. Between four to five convolutional/deconvolutional layers are used, depending on the domains used in $A$ and $B$ (we match the published code architecture per dataset). The discriminator is similar to the encoder, but has an additional convolutional layer as the first layer and a sigmoid output unit. 

The first set of experiments considers the CelebA face dataset. {\color{black}The results for hair color conversions are shown in} {\color{black} Fig.~\ref{fig:celebA_blond}}. It is evident that the output image is closely related to the input images, despite the fact that cycle loss terms were not used.

%\subsubsection{Empirical Validation of Prediction 2}

In Prediction 2, we predict that the selection of the right number of layers is crucial in unsupervised learning. Using fewer layers than needed, will not support the modeling of the target distribution. By contrast, adding superfluous layers would mean that more and more alternative mappings obscure the target transformation. 

In~\citep{pmlr-v70-kim17a}, 8 or 10 layers are employed  (counting both convolution and deconvolution), depending on the experiment. In our experiment, we vary the number of layers and inspect the influence on the results. 

{\color{black} To see the influence of the number of layers of the generator on the results, we employed the DiscoGAN~\citep{pmlr-v70-kim17a} public implementation and added or removed layers from the generator.}
{\color{black}The experiment was} done on the CelebA dataset for male to female conversion where 8 layers are employed in the experiments of~\citep{pmlr-v70-kim17a}. {\color{black}The results are illustrated in Fig.~\ref{fig:sw004}.} Note that since the encoder and the decoder parts of the learned network are symmetrical, the number of layers is always even. As can be seen, changing the number of layers has a dramatic effect on the results. The best results are obtained at 6 or 8 layers with 6 having the best alignment and 8 having better discrepancy. The results degrade quickly, as one deviates from the optimal value. Using fewer layers, the GAN fails to produce images of the desired class. Adding layers, the semantic alignment is lost, just as expected.

% {\color{black}To provide a numerical analysis, we employ the VGG descriptor~\citep{Parkhi15} to obtain a measure of both separation accuracy and discrepancy as the number of layers vary. We  check if the identity is preserved post mapping by comparing the VGG face descriptors. One can assume that two matching images will have many similar features and so the VGG representation will be similar. The cosine similarities are used, as is commonly done. As we can see, in the DiscoGAN experiments, the optimal values of the three measurements are obtained for 6 and 8 layers.}






% While our discrete notion of complexity seems to be highly related to the quality of the results, the norm of the weights do not seem to point to a clear architecture, as shown in Tab.~\ref{tab:a001}(a). Since the table compares the norms of architectures of different sizes, we also approximated the functions using networks of a fixed depth $k=18$ and then measured the norm. These results are presented in Tab.~\ref{tab:a001}(b). In both cases, the optimal depth, which is 6 or 8, does not appear to have a be an optimum in any of the measurements. 

% Prediction 3 states that there are only a handful of DPMs,  except for the identity function. In order to verify it, we trained a DiscoGAN from a distribution $A$ to itself with an added loss of the form $-\sum_{x\in A}|x-h(x)|$. In our experiment, testing network complexities from 2 to 12, we could not find a DPM, see Fig.~\ref{fig:c001} and Tab.~\ref{tab:c001}. For lower complexities, the identity was learned despite the added loss. For higher complexities, the network learned the identity while changing the background color. For even higher complexities, other mapping emerged. However, these mappings did not satisfy the circularity constraint, and are unlikely to be DPMs.
% SAY SOMETHING ABOUT CHANGING BACKGROUND COLOR OF IDENTITYE -> Style Transfer -> More complicated geometric transformation. 




\subsection{Results for Algs.~\ref{algo:when} and~\ref{algo:rtrvl}}


\begin{figure*}[t]
\centering
\hspace{-0.6cm}
  \begin{tabular}{c@{~}c@{~}c}
  \centering{\begin{turn}{90}\;\;\;\;~~~Shoes2Edges\end{turn}}&\includegraphics[width=0.4\linewidth, clip]{figures_per_epoch/shoes_disco_per_epoch.pdf}&%\hspace{-0.4cm} 
\includegraphics[width=0.4\linewidth, clip]{figures_per_epoch/shoes_dist_per_epoch.pdf}\\
& (Alg~\ref{algo:when}, discoGAN)  & (Alg~\ref{algo:when}, distanceGAN) \\
\end{tabular}
\caption{{\color{black}Results of Alg.~\ref{algo:when} for mapping Shoes to Edges. Ground truth errors are in red and bound in black. x-axis is the iteration. y-axis is expected risk. It takes a few epochs for $h_1$ to have a small enough discrepancy, until which the bound is ineffective.}}
  \label{fig:whenMain}
\end{figure*}

We test the two algorithms on two unsupervised alignment methods: DiscoGAN~\citep{pmlr-v70-kim17a} and % CycleGAN~\cite{CycleGAN2017}, and 
DistanceGAN~\citep{distgan}. In DiscoGAN, we train $h_1$ (and $h_2$), using two GANs and two circularity constraints; in DistanceGAN, {\color{black}to train $h_1$ (and $h_2$),} one GAN and one distance correlation loss are used. The published hyperparameters for each dataset are used, except when using Hyperband, where we vary the {\color{black}number of layers, the} learning rate and the batch size. 

Five datasets were used in the experiments: (i) aerial photographs to maps, trained on data scraped from Google Maps~\citep{pix2pix}, (ii) the mapping between photographs from the cityscapes dataset and their per-pixel semantic labels~\citep{Cordts2016Cityscapes}, (iii) architectural photographs to their labels from the CMP Facades dataset~\citep{facades},  (iv) handbag images~\citep{handbag} to their binary edge images, as obtained from the HED edge detector~\citep{hed}, and (v) a similar dataset for the shoe images from~\citep{shoes}.

Throughout the experiments, fixed values are used as the low-discrepancy threshold ($\epsilon_0=0.2$). The tradeoff parameter between the dissimilarity term and the fitting term during the training of $h_2$ is set, per dataset, to be the maximal value, such that the fitting of $h_2$ provides a solution that has a discrepancy lower than the threshold. This is done once, for the default parameters of $h_1$, as given in the original DiscoGAN and DistanceGAN~\citep{pmlr-v70-kim17a,distgan}.

The results of all experiments are summarized in Tab.~\ref{tab:mainresults}, which presents the correlation and p-value between the ground truth error, as a function of the independent variable, and the bound. The independent variable is either the training epoch or the sample, depending on the algorithm tested. For example, in Alg.~\ref{algo:when} we wish to decide on the best epoch, the independent variable is the training epoch. A high correlation (low p-value) between the bound and the ground truth error, both as a function of the number of layers, indicates the validity of the bound and the utility of the algorithm. Similar correlations are shown with the GAN losses and the reconstruction losses (DiscoGAN) or the distance correlation loss (DistanceGAN), in order to demonstrate that these are much less correlated with the ground truth error. In Fig.~\ref{fig:whenMain}, we omit the other scores in order to reduce clutter.

\begin{table*}[t]
\centering
\begin{small}
\caption{Pearson correlations and the corresponding p-values (in parentheses) of the ground truth error with: (i) the bound, (ii) the GAN losses, and (iii) the circularity losses or (iv) the distance correlation loss. %Note that the p-value is a function of both the correlation strength and the number of samples, which is larger for Alg.~2. 
$^{*}$The cycle loss $A\rightarrow B\rightarrow A$ is shown for DiscoGAN and the distance correlation loss is shown for DistanceGAN.}
\label{tab:mainresults}
\resizebox{0.99000995\textwidth}{!}{% <------ Don't forget this %
\begin{tabular}{l@{~~}l@{~~}llcccc}
\toprule
Alg. & Method & Dataset & Bound & $GAN_A$ & $GAN_B$ & $Cycle_A/\mathcal{L}_D$$^{*}$ & $Cycle_B$ \\
\midrule

Alg.~\ref{algo:when}  & Disco-    & Shoes2Edges    & {\bf 1.00} (\textless1E-16)          & -0.15 (3E-03)         & -0.28 (1E-08)  & 0.76(\textless1E-16)           & 0.79(\textless1E-16)   \\
                             &  GAN~\cite{pmlr-v70-kim17a}          &&&&&\\ %& Bags2Edges &        {\bf 1.00}	(\textless1E-16)& -0.26 (6E-11) &	-0.57 (\textless1E-16) &	0.85 (\textless1E-16) &	0.84 (\textless1E-16)           \\
                             %&             & Cityscapes        & {\bf 0.94}   (\textless1E-16)        & -0.66 (\textless1E-16)          & -0.69 (\textless1E-16)          & -0.26  (1E-07)        & 0.80 (\textless1E-16)   \\
                             %&             & Facades           & {\bf 0.85}  (\textless1E-16)         & -0.46  (\textless1E-16)        & 0.66 (\textless1E-16)           & 0.92 (\textless1E-16)          & 0.66  (\textless1E-16)         \\
                             %&             & Maps              & {\bf 1.00}     (\textless1E-16)      & -0.81 (\textless1E-16)          & 0.58  (\textless1E-16)         & 0.20   (9E-05)        & -0.14   (5E-03)       \\
                             %& Distance- & Shoes2Edges    &           {\bf 0.98} (\textless1E-16)	& - &	-0.25	(2E-16) & -0.14 (1E-05)	    &       -         \\
                             %&  GAN~\cite{distgan}           & Bags2Edges &            {\bf 0.93} (\textless1E-16) & - &	-0.08 (2E-02) &	0.34	(\textless1E-16)     &        -        \\
                             
                             %&             & Cityscapes        & {\bf 0.59}  (\textless1E-16)         & -          & 0.22   (1E-11)        & -0.41   (\textless1E-16)        &          -      \\
                             %&             & Facades           & {\bf 0.48}    (\textless1E-16)       & -        & 0.03  (5E-01)         & -0.01   (9E-01)       &        -        \\
                             %&             & Maps              & {\bf 1.00}    (\textless1E-16)       & -         & -0.73  (\textless1E-16)         & 0.39   (4E-16)        &      -          \\


\midrule
Alg.~\ref{algo:where} & Disco-    & Shoes2Edges    & {\bf 0.92}  (\textless1E-16)         & -0.12 (5E-01)         & 0.02  (9E-01)         & 0.29  (6E-02)         & 0.15    (4E-01)       \\
                             &       GAN~\cite{pmlr-v70-kim17a}      & Bags2Edges & {\bf 0.96}  (\textless1E-16)           & 0.25  (1E-01)         & 0.08   (6E-01)        & 0.08   (6E-01)        & 0.05  (7E-01)         \\
                             &             & Cityscapes        &        {\bf 0.78} (4E-04) &	0.24 (4E-01)	& -0.16 (6E-01) &	-0.04 (9E-01) &	0.03 (9E-01)    \\
                             &             & Facades           & {\bf 0.80}   (6E-10)        & 0.13   (4E-01)        & 0.16     (3E-01)      & 0.20    (2E-01)       & 0.09     (5E-01)      \\
                             &             & Maps             & {\bf 0.66}    (1E-03)       & 0.08   (7E-01)        & 0.12    (6E-01)       & 0.17   (5E-01)        & -0.25  (3E-01)        \\
                             & Distance- & Shoes2Edges    & {\bf 0.98}    (\textless1E-16)        & -     & -0.05   (7E-01)       & 0.84  (\textless1E-16)         & -               \\
                             &     GAN~\cite{distgan}        & Bags2Edges &  {\bf 0.92}      (\textless1E-16)      & -        & -0.28  (2E-01)        & 0.45    (3E-02)       &         -       \\
                             &             & Cityscapes        &   {\bf 0.51} (4E-04)            &        -        &   0.10 (5E-01)             &        0.28 (2E-2)        &           -     \\
                             &             & Facades           & {\bf 0.72}    (\textless1E-16)        & -      & -0.01    (1E00)      & 0.08  (6E-01)         &   -        \\
                             &             & Maps              &  {\bf 0.94}   (1E-06)        & -    & 0.20    (2E-01)       & 0.30  (6E-02)          &       -  \\
%1    & DiscoGAN & Facades     & %\ref{fig:somefig}(a) & 
%{{\bf \begin{tabular}[c]{@{}l@{}}0.77\\ 2.2E-6\end{tabular}}} & \begin{tabular}[c]{@{}l@{}}0.27\\ 1.2E-1\end{tabular}          &         &     %      &           \\
\bottomrule
\end{tabular}}
\end{small}
\end{table*}



\paragraph{Stopping Criterion (Alg.~\ref{algo:when})} For testing the stopping criterion suggested in Alg.~\ref{algo:when}, we compared, at each time point, two scores that are averaged over all training samples: $\|h_1(x) - h_2(x)\|$, which is our bound in Eq.~\ref{eq:boundEps0} (excluding the $+\epsilon_0$ term), and the ground truth error $\|h_1(x) - y(x)\|$, where $y(x)$ is the ground truth image that matches $x$ in domain $B$. 

The results are depicted in the main results table (Tab.~\ref{tab:mainresults}) as well as in Fig.~\ref{fig:whenMain} for both DiscoGAN (first column) and DistanceGAN (second column). {\color{black} The results for Shoes to Edges are depicted in Fig.~\ref{fig:whenMain}.} As can be seen, there is an excellent match between the mean ground truth error of the learned mapping $h_1$ and the predicted error. No such level of correlation is present when considering the GAN losses or the reconstruction losses (for DiscoGAN), or the distance correlation loss of DistanceGAN. Specifically, the very low p-values in the first column of Tab.~\ref{tab:mainresults} show that there is a clear correlation between the ground truth error and our bound for all datasets. For the other columns, the values in question are chosen to be the losses used for $h_1$. The lower scores in these columns show that none of these values are as correlated with the ground truth error, and so cannot be used to estimate this error.

In the experiment of Alg.~\ref{algo:when} for DiscoGAN, which has a large number of sample points, the cycle from $B$ to $A$ and back to $B$ is significantly correlated with the ground truth error with very low p-values in four out of five datasets. However, its correlation is significantly lower than that of our bound.

{\color{black} These results also demonstrate the tightness of the bound in Thm.~\ref{thm:corBoundGEN}. As can be seen, the bound is tight (close to the test error) and highly correlated with the test error.}



\paragraph{Selecting Architecture with the Modified Hyperband Algorithm} Our bound is used in Sec.~\ref{sec:hyperband} to create an unsupervised variant of the Hyperband method. In addition to selecting the architecture, this allows for the optimization of multiple hyperparameters at once, while enjoying the efficient search strategy of the Hyperband method~\citep{hyperband}. 

Fig.~\ref{fig:hyperband} demonstrates the applicability of our unsupervised Hyperband-based method for different datasets, employing both DiscoGAN and DistanceGAN. The graphs show the error and the bound obtained for the selected configuration after up to 35 Hyperband iterations. As can be seen, in all cases, the method is able to recover a configuration that is significantly better than what is recovered, when only optimizing for the number of layers. To further demonstrate the generality of our method, we applied it on the UNIT~\citep{liu2017unsupervised} architecture. Specifically, for DiscoGAN and DistanceGAN, we optimize the number of encoder and decoder layers, batch size and learning rate, while for UNIT, we optimize for the number of encoder and decoder layers, number of resnet layers and learning rate. Fig.~\ref{fig:hyperband_unit} and Tab.~\ref{fig:hyperband}(b) show the convergence on the Hyperband method. 

\begin{figure*}[t]
\begin{tabular}{c@{~}c}
\multicolumn{2}{c}{\includegraphics[width=1.0\linewidth, clip]{graphs_hyperband/units_maps.pdf}}\\
~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~(a) & ~~~~(b)\\
\end{tabular}
\caption{{\color{black} Applying unsupervised Hyperband for selecting the best configuration for UNIT for the Maps dataset. The $x$-axis is the iteration count and the $y$-axis is the error/bound value of the selected configuration. (a) blue and orange lines are bound and ground truth error as in Fig.~\ref{fig:hyperband}. (b) Images produced for three different configurations, as indicated on the plot in (a).} }
 \label{fig:hyperband_unit}
\end{figure*}

\begin{figure*}[t]
\centering
  %\begin{tabular}{ccccc}
%\hspace{-0.4cm}\includegraphics[width=0.20\linewidth, clip]{graphs_hyperband/maps_new.png}&
%\includegraphics[width=0.20\linewidth, clip]{graphs_hyperband/cityscapes_new.png}&
%\includegraphics[width=0.20\linewidth, clip]{graphs_hyperband/facades_new.png}&
% \includegraphics[width=0.20\linewidth, clip]{graphs_hyperband/shoes_new.png}&
%  \includegraphics[width=0.20\linewidth, clip]{graphs_hyperband/handbags_new.png}\\
%\hspace{-0.4cm}\includegraphics[width=0.20\linewidth, clip]{graphs_hyperband/distance_maps_new.png}&
%\includegraphics[width=0.20\linewidth, clip]{graphs_hyperband/distance_cityscapes_new.png}&
% TODO!!!
%\includegraphics[width=0.20\linewidth, clip]{graphs_hyperband/distance_cityscapes_new.png}&
% \includegraphics[width=0.20\linewidth, clip]{graphs_hyperband/distance_shoes_new.png}&
 % \includegraphics[width=0.20\linewidth, clip]{graphs_hyperband/distance_handbags_new.png}\\
 
 %(Maps) & (Cityscapes) & (Facades) & (Shoes2Edges) & (Handbags2Edges)\\
%\end{tabular}
\vspace{-2cm}
\begin{minipage}{0.656772\textwidth}
\centering
\begin{tabular}{c@{~}c@{~}c}
\centering{\begin{small}\begin{turn}{90}\;\;\;\;\;\; \hspace{3mm} Maps\end{turn}\end{small}}&
\includegraphics[width=0.482\linewidth, clip]{graphs_hyperband/maps_new.png}\vspace{-2mm}&
\includegraphics[width=0.482\linewidth, clip]{graphs_hyperband/distance_maps_new.png}\vspace{-2mm}\\
\centering{\begin{small}\begin{turn}{90}\;\;\;\;\;\; \hspace{1mm}Cityscapes\end{turn}\end{small}}&
\includegraphics[width=0.482\linewidth, clip]{graphs_hyperband/cityscapes_new.png}\vspace{-2mm}&
\includegraphics[width=0.482\linewidth, clip]{graphs_hyperband/distance_cityscapes_new.png}\vspace{-2mm}\\

\centering{\begin{small}\begin{turn}{90}\;\;\;\;\;\; \hspace{3mm}Facades\end{turn}\end{small}}&
\includegraphics[width=0.482\linewidth, clip]{graphs_hyperband/facades_new.png}\vspace{-2mm}&
\includegraphics[width=0.482\linewidth, clip]{graphs_hyperband/distance_facades_new.png}\vspace{-2mm}\\
\centering{\begin{small}\begin{turn}{90}\;\;\;\;\;\; \hspace{-3mm} Bags2Edges\end{turn}\end{small}}&
\includegraphics[width=0.482\linewidth, clip]{graphs_hyperband/handbags_new.png}\vspace{-2mm}&
\includegraphics[width=0.482\linewidth, clip]{graphs_hyperband/distance_handbags_new.png}\vspace{-2mm}\\

\centering{\begin{small}\begin{turn}{90}\;\;\;\;\;\; Shoes2Edges\end{turn}\end{small}}&
\includegraphics[width=0.482\linewidth, clip]{graphs_hyperband/shoes_new.png}\vspace{-2mm}&
\includegraphics[width=0.482\linewidth, clip]{graphs_hyperband/distance_shoes_new.png}\vspace{-2mm}\\
 \multicolumn{3}{c}{(a)}
  \\
\end{tabular}
  \end{minipage}%
\begin{minipage}{.71\textwidth}
\hspace{0.1mm}
\begin{small}
\resizebox{0.48\textwidth}{!}{% <------ Don't forget this %
\begin{tabular}{l@{~~}ccc}
\toprule
Dataset & Number & Batch & Learning \\
 &  Layers & Size & Rate \\
\midrule
\multicolumn{4}{c}{DiscoGAN~\citep{pmlr-v70-kim17a}}\\
            Shoes2Edges       & 3 & 24 & 0.0008 \\
            Bags2Edges        & 2 & 59 &	0.0010 \\
                                  Cityscapes        & 3 & 27 & 0.0009 \\
                                  Facades           & 3 & 20 & 0.0008 \\
                                  Maps              & 3 & 20 & 0.0005 \\
                                  \multicolumn{4}{c}{DistanceGAN~\citep{distgan}} \\
                             Shoes2Edges       & 3 & 15 & 0.0007 \\
                Bags2Edges        & 3 & 33 &	0.0007 \\
                                  Cityscapes        & 4 & 21 & 0.0006 \\
                                  Facades           & 3 & 8  & 0.0006 \\
                                  Maps              & 3 & 20 & 0.0005 \\     
                                  \toprule
Dataset & \#Layers & \#Res & L.Rate \\
% & Layers & Layers & Rate \\
 \midrule
\multicolumn{4}{c}{UNIT~\citep{liu2017unsupervised}} \\
                                  Maps              & 3 & 1 & 0.0003 \\     
\bottomrule
%\hspace{0.1mm}
%& & &\\
\multicolumn{4}{c}{(b)}
\end{tabular}}
%\end{small}
%\end{minipage}%
%\begin{minipage}{0.656772\textwidth}

\centering
\hspace{0.3mm}
\begin{tabular}{l@{~~}l@{~~~}l}
& {\scriptsize default} & {\scriptsize unsupervised}\\
 & {\scriptsize parameters} & {\scriptsize hyperband} \\
~~~$x$ & {\footnotesize $h_1(x)$} & {\footnotesize $h_1(x)$} \\

\includegraphics[width=0.120\linewidth, clip]{images_hyperband_before/2_B.png}&
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_before/2_BA.png}&
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_after/2_BA.png} \\
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_before/3_B.png}&
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_before/3_BA.png}&
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_after/3_BA.png} \\
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_before/5_B.png}&
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_before/5_BA.png}&
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_after/5_BA.png} \\
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_before/13_B.png}&
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_before/13_BA.png}&
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_after/13_BA.png} \\
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_before/16_B.png}&
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_before/16_BA.png}&
\includegraphics[width=0.120\linewidth, clip]{images_hyperband_after/16_BA.png} \\
 \multicolumn{3}{c}{(c)}
  \\
\end{tabular}
\end{small}
  \end{minipage}%
% (b) \\ 
% \resizebox{0.99000995\textwidth}{!}{% <------ Don't forget this %
% \begin{tabular}{l@{~~}|c|ccc|c|ccc}
% \toprule
% Dataset & Method & Number of Layers & Batch Size & Learning Rate & Method & Number of Layers & Batch Size & Learning Rate \\
% \midrule
% Shoes2Edges &  Disco-       & 3 & 24 & 0.0008  & Dist-                           &  3 & 15 & 0.0007 \\
% Bags2Edges  &  GAN~\cite{pmlr-v70-kim17a}    & 2 & 59 &	0.0010 &   GAN~\cite{distgan}             & 3 & 33 &	0.0007 \\
% Cityscapes &        & 3 & 27 & 0.0009 & & 4 & 21 & 0.0006 \\
% Facades    &       & 3 & 20 & 0.0008 & &      &   &           \\
% Maps       &       & 3 & 20 & 0.0005 &  & 3 & 20 & 0.0005 \\   
% \bottomrule
% \end{tabular}} 
\caption{\small {\color{black}Applying unsupervised hyperband for selecting the best configuration. For DiscoGAN and DistanceGAN, we optimize of the number of encoder and decoder layers, batch size and learning rate, while for UNIT, we optmized for the number of encoder and decoder layers, number of resnet layers and learning rate. (a) For each dataset, the first plot is of DiscoGAN and the second is of DistanceGAN. Hyperband optimizes, according to the bound values indicated in blue. The corresponding ground truth errors are shown in orange. Dotted lines represent the best configuration errors, when varying only the number of layers without hyperband (blue for bound and orange for ground truth error). Each graph shows the error of the best configuration selected by hyperband, as a function the number of hyperband iterations. (b) The corresponding hyperparameters of the best configuration as selected by hyperband. (c) Images produced for DiscoGAN's shoes2edges: 1st column is the input, the 2nd is the result of DiscoGAN's default configuration, 3rd is the result of the configuration  selected by our unsupervised Hyperband.} }
  \label{fig:hyperband}
\end{figure*}



\paragraph{Predicting per-Sample loss with Alg.~\ref{algo:where}} Finally, we consider the per sample loss. %Determining the success of the prediction of a computer vision method for a given sample is often crucial, yet challenging even for supervised methods that predict a single value. 
The results are plotted in Fig.~\ref{fig:oneSamp2}. {\color{black}Each point in the plot specifies the evaluation of the bound ($y$-axis) vs. the per-sample error ($x$-axis) of the trained generator $h_1$ for a specific point $x$ in domain $A$. The numbered points in the graph correspond to the samples in (b).} As can be seen, there is a high degree of correlation {\color{black}(the coefficient of determination is large, $R^2=0.9145$)} between the measured bound and the ground truth error. Therefore, our method is {\color{black}a reliable predictor of} the per-sample success of a multivariate mapping learned in a fully unsupervised manner. 

\begin{figure*}[t]
  \centering
  \begin{tabular}{c@{~~~~~~~~~~}c}
\includegraphics[width=0.425\linewidth, clip]
{graphs_per_sample/handbags2edges_plot__2_.png}&
\includegraphics[width=0.24\linewidth, clip]{graphs_per_sample/images_edges2handbags_rr.png}\\
(a) & (b) \\
\end{tabular}
\caption{{\color{black} Results of Alg.~\ref{algo:where} on DiscoGAN for Handbags2Edges. (a) The ground truth errors ($x$-axis) vs. the bound per point ($y$-axis) are shown.
(b) The source ($x$), ground truth ($y(x)$) and mapping ($h_1(x)$) of the marked points.}}
\label{fig:oneSamp2}
\end{figure*}


\subsection{Results for Alg.~\ref{algo:duallayers}}


\begin{figure}[t]
    \centering
    \begin{minipage}{.5\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figures_dual/DUALmale2femaleS.pdf}
    \end{minipage}%
    \begin{minipage}{0.5\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figures_dual/DUALedges2shoesS.pdf}
    \end{minipage}
    \caption{\label{fig:dual} {\color{black} Results for Alg.~\ref{algo:duallayers} on Male2Female and Edges2Shoes datasets for mapping Male to Female (and for mapping Edges to Shoes, resp.). Shown are a minimal complexity mapping $g$ that has low discrepancy, and various mappings $h$ obtained by the method.}}
\end{figure}
 

The goal of Alg.~\ref{algo:duallayers} is to find a well-aligned solution with higher complexity than the minimal solution and a potentially smaller discrepancy. It has two stages. In the first one, $k_1$, which is the minimal complexity that leads to a low discrepancy, is identified. This follows a set of experiments that are similar to the one that is captured, for example, by Fig.~\ref{pred2}. To demonstrate robustness, we select a single value of $k_1$ across all experiments. Specifically, we use $k_1=6$, which, as discussed above, typically leads to a low (but not very low) discrepancy, while the alignment is still unambiguous.  

Once $g$ is trained, we proceed to the next step of optimizing a second network of complexity $k_2$. Note that while the first function ($g$) uses the complete DiscoGAN architecture, the second network ($h$) only employs a one-directional mapping, since alignment is obtained by $g$.

{\color{black}We conducted the experiments on the CelebA dataset for Male to Female and Edges to Shoes conversions. Fig.~\ref{fig:dual} depicts} the obtained results, for a varying number of layers. First, the result obtained by the DiscoGAN method with $k_1$ is displayed. The results of applying Alg.~\ref{algo:duallayers} are then displayed for a varying $k_2$.

As can be seen, our algorithm leads to more sophisticated mappings. \cite{pmlr-v70-kim17a} have noted that their solutions are, at many times, related to texture or style transfer and, for example, geometric transformations are not well-captured. The new method is able to better capture such complex transformations. Consider the case of mapping Male to Female in Fig.~\ref{fig:dual}, first row. A man with a beard is mapped to a female image. While for $g$ the beard is still somewhat present, it is not so for $h$ with $k_2>k_1$. For the Edges to Shoes {\color{black} mapping of Fig.~\ref{fig:dual}}, while the general structure is clearly present, it is significantly sharpened by mapping $h$ with $k_2>k_1$. 


